Using Linear Dynamical Topic Model for Inferring Temporal Social Correlation in Latent Space

The abundance of online user data has led to a surge of interests in understanding the dynamics of social relationships using computational methods. Utilizing users' items adoption data, we develop a new method to compute the Granger-causal (GC) relationships among users. In order to handle the high dimensional and sparse nature of the adoption data, we propose to model the relationships among users in latent space instead of the original data space. We devise a Linear Dynamical Topic Model (LDTM) that can capture the dynamics of the users' items adoption behaviors in latent (topic) space. Using the time series of temporal topic distributions learned by LDTM, we conduct Granger causality tests to measure the social correlation relationships between pairs of users. We call the combination of our LDTM and Granger causality tests as Temporal Social Correlation. By conducting extensive experiments on bibliographic data, where authors are analogous to users, we show that the ordering of authors' name on their publications plays a statistically significant role in the interaction of research topics among the authors. We also present a case study to illustrate the correlational relationships between pairs of authors.

==> latex/appendices.tex <==
\section*{APPENDIX}
\setcounter{section}{1}
\label{sec:appendix}

\begin{comment}
	\begin{pmatrix}
	\mu_{n,t,1} & \ldots & 0 & \ldots & 0 \\
	\vdots & \ddots & \vdots & \iddots  &  \vdots \\
	0 & \ldots & \mu_{n,t,k} & \ldots & 0 \\
	\vdots & \iddots & \vdots & \ddots & \vdots \\
	0 & \ldots & 0 & \ldots & \mu_{n,t,K} \\ 
	\end{pmatrix}
\end{comment}

\[ A_{n,t} = \begin{pmatrix} \mu_{n,t,1} & & \\ & \mu_{n,t,k} & \\ & & \mu_{n,t,K} \end{pmatrix} \]
Assume that the dynamics matrix $A_{n,t}$ is a diagonal matrix with entries $\{ \mu_{n,t,1},\ldots,\mu_{n,t,K} \}$. We express the individual components of Equation \ref{eqn:gradient_mu} from Section \ref{sec:estimate_dynamics}. The same equation is also shown here for easy reference:

{\small \[ \frac{d \mathcal{L}}{d \mu_{n,t-1,k}} = \frac{d E \left( \theta_{n,t,k|t} \right) }{d \mu_{n,t-1,k}} \left[ \log \frac{ E \left( \theta_{n,t,k|t} \right) } { E \left( \theta_{n,t,k|t-1} \right) } \right] + E \left( \theta_{n,t,k|t} \right) \left[ \frac{d \log E \left( \theta_{n,t,k|t} \right) }{d \mu_{n,t-1,k}} - \frac{d \log E \left( \theta_{n,t,k|t-1} \right) }{d \mu_{n,t-1,k}} \right] \] }

Use the following equations:
\begin{gather*}
	E \left( \theta_{n,t,k|t-1} \right) = \frac{ \mu_{n, t-1, k} \cdot x_{n,t-1,k|t-1} + \alpha }{ 1' A_{n, t-1} \cdot x_{n,t-1|t-1} + K \alpha } \quad
	E \left( \theta_{n,t,k|t} \right) = \frac{ \mu_{n, t-1, k} \cdot x_{n,t-1,k|t-1} + \psi_{n, t, k} + \alpha }{ 1' \left( A_{n, t-1} \cdot x_{n,t-1|t-1} + \psi_{n, t} \right) + K \alpha } \\
\end{gather*}
\begin{align*}
	\frac{d E \left( \theta_{n,t,k|t} \right) }{d \mu_{n,t-1,k}} &= \frac{ x_{n,t-1,k|t-1} \left( 1' \psi_{n, t} + K \alpha \right) - 1' x_{n,t-1|t-1} \left( \psi_{n, t, k} + \alpha \right) }{ \left[ 1' \left( A_{n, t-1} \cdot x_{n,t-1|t-1} + \psi_{n, t} \right) + K \alpha \right]^2 } \\
	\frac{d \log E \left( \theta_{n,t,k|t} \right) }{d \mu_{n,t-1,k}} &= \frac{1}{E \left( \theta_{n,t,k|t} \right)} \frac{d E \left( \theta_{n,t,k|t} \right) }{d \mu_{n,t-1,k}} \\
	\frac{d \log E \left( \theta_{n,t,k|t-1} \right) }{d \mu_{n,t-1,k}} &= \frac{x_{n,t-1,k|t-1}}{\mu_{n,t-1,k} \cdot x_{n,t-1,k|t-1} + \alpha} - \frac{1' x_{n,t-1|t-1}}{1' A_{n, t-1} \cdot x_{n,t-1|t-1} + K \alpha}
\end{align*}



